Differentially Private Empirical Cumulative Distribution Functions

In order to both learn and protect sensitive training data, there has been a growing interest in privacy preserving machine learning methods. Differential privacy has emerged as an important measure of privacy. We are interested in the federated setting where a group of parties each have one or more training instances and want to learn collaboratively without revealing their data. In this paper, we propose strategies to compute differentially private empirical distribution functions. While revealing complete functions is more expensive from the point of view of privacy budget, it may also provide richer and more valuable information to the learner. We prove privacy guarantees and discuss the computational cost, both for a generic strategy fitting any security model and a special-purpose strategy based on secret sharing. We survey a number of applications and present experiments.

==> related_work.tex <==

\section{Related Work}
\label{sec:related}

Strategies to compute secure averages can be built depending on the level of trust put in the aggregator or in the users, on the utility and the verifability of results and lastly on the level of communication overhead.
Local differential privacy (LDP) \cite{Kasiviswanathan2008,d13,kairouz2015secure,Kairouz2016a,discrete_dis_local} does not require to trust the aggregator or users but brings litte utility and no verifability. The use of cryptographic primitives combined with DP \cite{pmlr-v139-kairouz21a,skellam} allows exact aggregation but is not verifiable, except \cite{Dwork2006ourselves}. It requires $\Omega(n)$ communication per party and does not reflect the impact of colluding/malicious users except \cite{Jayaraman2018} which relies on two non-coluding servers. Recently the shuffle model of privacy \cite{Cheu2019,amp_shuffling,Hartmann2019,Balle2020,Ghazi2020ICML} assumes honest-but-curious parties with high communication overhead but can match the utility of the trusted curator model. Lastly, the use of correlated Gausian noise \cite{imtiaz2021distributed, sabater2021accurate} can have utility of central models but only \cite{sabater2021accurate} can do it with malicious users and with only $O(\log n)$ communication.

